FAIR: A Causal Framework for Accurately Inferring Judgments Reversals

Artificial intelligence researchers have made significant advances in legal intelligence in recent years. However, the existing studies have not focused on the important value embedded in judgments reversals, which limits the improvement of the efficiency of legal intelligence. In this paper, we propose a causal Framework for Accurately Inferring case Reversals (FAIR), which models the problem of judgments reversals based on real Chinese judgments. We mine the causes of judgments reversals by causal inference methods and inject the obtained causal relationships into the neural network as a priori knowledge. And then, our framework is validated on a challenging dataset as a legal judgment prediction task. The experimental results show that our framework can tap the most critical factors in judgments reversal, and the obtained causal relationships can effectively improve the neural network's performance. In addition, we discuss the generalization ability of large language models for legal intelligence tasks using ChatGPT as an example. Our experiment has found that the generalization ability of large language models still has defects, and mining causal relationships can effectively improve the accuracy and explain ability of model predictions.

==> ref.tex <==

% 参考文献





% Legal Intelligence
Legal Judgment Prediction via Event Extraction with Constraints
EPM
% 带有事件之间的约束条件的LJP模型

Exploiting Contrastive Learning and Numerical Evidence for Improving
Confusing Legal Judgment Prediction
NSCL
% 对比学习，学习法条之间的细微差异， LJP

Iteratively Questioning and Answering for Interpretable Legal Judgment Prediction
QAjudge
% LJP引入强化学习

Lawformer: A pre-trained language model for Chinese legal long documents
% 为法律领域长文本设计的预训练模型

CAIL2018: A Large-Scale Legal Dataset for Judgment Prediction
%判决预测的大规模中国法律数据集

LEVEN: A Large-Scale Chinese Legal Event Detection Dataset
% 法律事件检测数据集

Swiss-Judgment-Prediction: A Multilingual Legal Judgment Prediction Benchmark.
FSCS
% 多语言LJP数据集

LeSICiN: A Heterogeneous Graph-Based Approach for Automatic Legal Statute Identification from Indian Legal Documents
% 法律法规识别任务

Legal Judgment Prediction with Multi-Stage Case Representation Learning in the Real Court Setting
MSJudge
% 法庭辩论的多角色对话场景的LJP
%这些Legal dataset没有注意改判问题，因此没有提供所需要的改判信息，所以本文的数据集是自己找的



% Casusal Inference for Legal domain
Everything Has a Cause: Leveraging Causal Inference in Legal Text Analysis
% 法律领域无监督text因果推断

%Counterfactuals for causal responsibility in legal contexts
%Andreas
%基于反事实的方法为法律背景下的责任归属问题提供了解决方案

A normative model of explanation for binary classification legal AI and its implementation on causal explanations of Answer Set Programming
Evan
%使用因果推断为法律实践中的二进制算法提供解释性

Law Article-Enhanced Legal Case Matching: a Model-Agnostic Causal Learning Approach
Law-Match
% 运用因果推断将法律条款嵌入到法律案件匹配任务

Knowledge is Power: Understanding Causality Makes Legal judgment Prediction Models More Generalizable and Robust
% 引入因果推断消除LJP任务中的伪相关误差

Causal Models of Legal Cases
Liepina
% 介绍了一个半正式的因果推理框架来模拟法律案件中的事实因果关系论证

Causal analysis for attributing responsibility in legal cases
Chockler
% 专注于法律责任归属问题，使用因果推断来捕捉多方和事件之间复杂的因果关系


%15



%intro ref

% 丰富的法律资源
LexGLUE: A Benchmark Dataset for Legal Language Understanding in English.

Neural Legal Judgment Prediction in English

JEC-QA: A Legal-Domain Question Answering Dataset.

% 任务
% LJP
Predicting the Law Area and Decisions of French Supreme Court Cases
% 匹配
Explainable Legal Case Matching via Inverse Optimal Transport-based Rationale Extraction
% 抽取
Joint Entity and Relation Extraction for Legal Documents with Legal
Feature Enhancement


% 21


ZLPR: A NOVEL LOSS FOR MULTI-LABEL CLASSIFICATION

%Label Smoothing
Rethinking the Inception Architecture for Computer Vision

DoWhy: Addressing Challenges in Expressing and Validating Causal Assumptions.

BERT：Pre-training of Deep Bidirectional Transformers for Language Understanding

https://openai.com/blog/chatgpt

https://www.pkulaw.com


Visualizing Data using t-SNE

% 26
